Fusing the Old with the New: Learning Relative Camera Pose with Geometry-Guided Uncertainty

Learning methods for relative camera pose estimation have been developed largely in isolation from classical geometric approaches. The question of how to integrate predictions from deep neural networks (DNNs) and solutions from geometric solvers, such as the 5-point algorithm, has as yet remained under-explored. In this paper, we present a novel framework that involves probabilistic fusion between the two families of predictions during network training, with a view to leveraging their complementary benefits in a learnable way. The fusion is achieved by learning the DNN uncertainty under explicit guidance by the geometric uncertainty, thereby learning to take into account the geometric solution in relation to the DNN prediction. Our network features a self-attention graph neural network, which drives the learning by enforcing strong interactions between different correspondences and potentially modeling complex relationships between points. We propose motion parmeterizations suitable for learning and show that our method achieves state-of-the-art performance on the challenging DeMoN and ScanNet datasets. While we focus on relative pose, we envision that our pipeline is broadly applicable for fusing classical geometry and deep learning.

==> Section/_BACKUP_method.tex <==
\section{Method}
\label{sec:method}
\subsection{Motivation: Limitation of Geometrical Solver}
Despite its well-established theoretical foundation, the classical geometrical solvers still face various challenges and our paper purports to leverage CNN for more accurate estimation under such cases.

\noindent \textbf{Correspondences}. The correspondence between two views have been the cornerstone of the geometrical solvers ever since. This heavy reliance on correspondences yet indicates degraded performance under the scarcity of correspondences.

\noindent \textbf{Degenearacy}. The geoemtric performance also drops when it approaches inherently degenerate configurations. One typical example is when most of the keypoints lie on a certain 3D plane. 

\noindent \textbf{Rotation vs. Translation}.
It is widely known~\cite{nister2004efficient,tian1996comparison} that translation estimates are far more sensitive than rotation; various issues in SfM are related to translation such as the familiar forward motion bias ~\cite{nister2004efficient} in linear methods if proper normalization is not carried out. Thus, one would naturally like to trust the rotation solution more in the geometric solution, whereas expect CNN to play a more significant role in the translation. We shall show that our uncertainty-based framework lends itself well to this purpose in a principled way.

\noindent \textbf{Bas-relief Ambiguity}. Bas-relief ambiguity~\cite{daniilidis1997understanding}, a.k.a. rotation translation ambiguity, rears its ugly head once the camera is undergoing sideway motion. This is due to the resemblance between translational and rotational flow under limited field of view, such confouding resulting in difficulty to distinguish one from the other and hence less accurate pose estimation.

\noindent \textbf{Forward Motion}. Forward motion also constantly pose challenges to SfM, partially because of the vanishing feature movement near the focus of expension at image center, and partially because of the presence of a plethora of local minima in the least squares error landscape~\cite{vedaldi2007moving,oliensis2005least}.


\subsection{Geometric Uncertainty}
\noindent \textbf{Geometric solution}. Formally, we are interested in solving the relative camera pose between two cameras $C_1$ and $C_2$ with known intrinsics. Specifically, taking $C_1$ as the reference with camera pose denoted as $\boldsymbol{P}_1=[\boldsymbol{I}~~\boldsymbol{0}]$, the problem is defined as solving the relative camera pose of $C_2$, denoted as $\boldsymbol{P}_2=[\boldsymbol{R}~~\boldsymbol{t}]$, where $\boldsymbol{R} \in SO(3)$ and $t\in S^2$ denote the relative rotation and translation direction, respectively. Suppose both camears are viewing a set of common 3D points $\boldsymbol{X}_i$, $i=1,2,...,n$, each yielding a pair of 2D correspondences $\boldsymbol{x}_i^1$ and $\boldsymbol{x}_i^2$ in the image plane. It is well-known that a minimal set of 5-point correspondences suffices to determine the solution, with Nister's 5-point algorithm~\cite{nister2004efficient} being the standard minimal solver. A RANSAC~\cite{fischler1981random} procedure is usually applied to obtain an initial solution, and triangulation~\cite{hartley2003multiple} follows to obtain 3D points $\boldsymbol{X}_i$. Finally, one could refine the solution by nonlinearly minimizing the reprojection error, a.k.a. bundle adjustment~\cite{triggs1999bundle},
\begin{equation}
    \min_{\boldsymbol{\theta}}\sum_{i}\|\boldsymbol{x}_i^1-\pi(\boldsymbol{P}_1,\boldsymbol{X}_i))\|^2+\|\boldsymbol{x}_i^2-\pi(\boldsymbol{P}_2,\boldsymbol{X}_i))\|^2,
    \label{eq:ba}
\end{equation}
where $\pi()$ denotes the standard perspective projection and  $\boldsymbol{\theta}=\{\boldsymbol{\theta}_R,~\boldsymbol{\theta}_t,\boldsymbol{X}_i, i=1,2,...n\}$. $\boldsymbol{\theta}_R$ and $\boldsymbol{\theta}_t$ represent the parameterization of rotation and translation; we will come back to their specific choice in next section.

\noindent \textbf{Uncertainty}. In order to describe the uncertainty associated with the optimum $\hat{\boldsymbol{\theta}}$ in a probabilistic manner, the distribution of $\boldsymbol{\theta}$ could be approximated locally by a Gaussian distribution $\mathcal{N}(\boldsymbol{\theta}|\hat{\boldsymbol{\theta}},\boldsymbol{\Sigma})$. As a first-order approximation, the information matrix \boldsymbol{\Lambda}, i.e. $\boldsymbol{\Sigma}^{-1}$, is commonly computed via Jacobian, i.e.,
\begin{equation}
    \boldsymbol{\Lambda}=J^\top(\hat{\boldsymbol{\theta}})J(\hat{\boldsymbol{\theta}}),
\end{equation}
where $J(\hat{\boldsymbol{\theta}})$ denotes the Jacobian of the nonlinear least squares (Eq.~\ref{eq:ba}) at $\hat{\boldsymbol{\theta}}$. We remark that $J(\hat{\boldsymbol{\theta}})$ is of full rank in this paper, implying the absence of gauge ambiguity~\cite{}. This is attributed to the fixed camera pose of $C_1$ as well as our minimal parameterizations of $(\boldsymbol{R},\boldsymbol{t})$ to be discussed shortly. In addition, we shall conduct fusion on each individual parameter in $\{\boldsymbol{\theta}_R,~\boldsymbol{\theta}_t\}$ separately due to the discontinuity in representation, and we shall work on inverse variance for convenience. To proceed, the inverse variance $\sigma_i^{-1}$ of a parameter $\theta_i$ in $\{\boldsymbol{\theta}_R,~\boldsymbol{\theta}_t\}$ could be obtained by Schur complement
\begin{equation}
    \sigma_i^{-1} = \boldsymbol{\Lambda}\setminus\boldsymbol{\Lambda}_{J,J} = \boldsymbol{\Lambda}_{i,i} - \boldsymbol{\Lambda}_{i,J}\boldsymbol{\Lambda}_{J,J}^{-1}\boldsymbol{\Lambda}_{J,i},
\end{equation}
where $J$ includes the index to all the rest parameters in $\boldsymbol{\theta}$. This step is also called S-transformation~\cite{baarda1973s} that purports to specify the gauge of covariance matrix~\cite{forstner2016photogrammetric,polic2020uncertainty}. From the probabilistic point of view, it is essentially the conditional variance of $\theta_i$ given all the other parameters~\cite{johnson2002applied}. The block sparsity of Jacobian is leveraged for efficient computation, as deatiled in the supplementary.

As readers might notice, we do not consider the keypoint localization uncertainty of $\boldsymbol{x}_i^{1,2}$ in this paper for the sake of simplicity.





\subsection{Geometric-CNN Pose fusion via Uncertainty}

\begin{figure*}[t]
	\centering
		\includegraphics[width=1.0\linewidth, trim = 0mm 15mm 0mm 0mm, clip]{Figure/pipeline.pdf}
	\centering
	\caption{Overview of our geometric-CNN pose fusion framework.}
	\label{fig:pipeline}
\end{figure*}






\noindent \textbf{Overview}. The overall framework of our geometry-CNN pose fusion pipeline is illustrated in Fig.~\ref{}. Our method takes as input the image pair along with the correspondences extrated by a feature extractor and matcher; in this paper, we make use of SuperPoint~\cite{} and SuperGlue~\cite{} due to their excellent performance. The two images are stacked and passed to a ResNet~\cite{} architecture to extract the appearance feature. The corresponding keypoint locations are feed into an attentional graph neural network to extract the geometric feature. Afterwards, the appearance and geometric features are concatenated before passed to the pose branch and the uncertainty branches, which predict the mean and inverse variance of the underlying Gaussian distribution of the motion parameters, via a Multilayer Perceptron (MLP). These are then fused with the geometric solution based on uncertainty, yielding the final output that receives the supervision signal.

\noindent \textbf{Motivation}. We would like to highlight the significance of the ResNet in that it offers the global appearance context for network to reason about the camera motion. This is very much complementary to traditional geometric approaches that only rely on keypoint correspondences, if available at all. The ResNet is admittedly pretty generic, however we leave the exploration of more specially tailored networks as future work since our contributions are orthogonal to the choice of appearance backbone. The purposes of our graph neural network and geometric feature are two-fold. First, the correspondences, if available, do encode strong geometric cues that could be leveraged by network to reason about camera motion. Second, as opposed to appearance, correspondences as the sole input to the 5-point solver and BA, have a more explicit correlation with the uncertainty of geometric solution. This facilitates the network to decide the extent to which the geometric solution should be trusted.


\noindent \textbf{Probabilistic Geometric-CNN Pose Fursion}. In order to fuse the geometric and CNN predictions, one could conceptually treat them as measurements from two different sensors, which leads to the natural application of traditional sensor fusion strategies---a principled way to sensor fusion is by the means of Bayes Law akin to kalman filter. Specifically, the posterior of a motion parameter $\boldsymbol{\theta}_i$ reads
\begin{equation}
    P(\boldsymbol{\theta}_i|\hat{\boldsymbol{\theta}}_{g,i},{\sigma}_{g,i},\hat{\boldsymbol{\theta}}_{c,i},{\sigma}_{c,i}) \propto P(\boldsymbol{\theta}_i) \mathcal{N}(\boldsymbol{\theta}_i|\hat{\boldsymbol{\theta}}_{g,i},{\sigma}_{g,i}) \mathcal{N}(\boldsymbol{\theta}_i|\hat{\boldsymbol{\theta}}_{c,i},{\sigma}_{c,i}),
\end{equation}
where $(\boldsymbol{\theta}_{g,i},\sigma_{g,i})$ and $(\boldsymbol{\theta}_{c,i},{\sigma}_{c,i})$ respectively denote the geometric and CNN prediction.
Assuming non-informative prior $P(\boldsymbol{\theta}_i)$, it can be shown that
\begin{equation}
P(\boldsymbol{\theta}_i|\hat{\boldsymbol{\theta}}_{g,i},{\sigma}_{g,i},\hat{\boldsymbol{\theta}}_{c,i},{\sigma}_{c,i}) = \mathcal{N}(\boldsymbol{\theta}_i|\hat{\boldsymbol{\theta}}_{f,i},\sigma_{f,i}),
\end{equation}
\begin{equation}
\hat{\boldsymbol{\theta}}_{f,i} = \frac{\sigma_{g,i}^{-1}\hat{\boldsymbol{\theta}}_{g,i} +\sigma_{c,i}^{-1}\hat{\boldsymbol{\theta}}_{c,i}}{\sigma_{g,i}^{-1}+\sigma_{c,i}^{-1}},~~\sigma_{f,i} =(\sigma_{g,i}^{-1}+\sigma_{c,i}^{-1})^{-1}.    
\end{equation}
It follows that $\hat{\boldsymbol{\theta}}_{f,i}$ is the maximum-a-posterior (MAP) estimator after fusion. One observes that it essentially boils down to a weighted average depending upon the confidence (inverse variance) of each prediction.  

\subsubsection{Motion parameterization}
\label{sec:motionparameter}
Here, we discuss various subtleties to choose the proper motion parameterizaton. 

\noindent \textbf{Translation}. We consider for translation direction the following two distinct parameterizations, 
\begin{equation}
    \boldsymbol{t}(t_x,t_y,t_z) = \frac{[t_x,t_y,t_z]^\top}{\|[t_x,t_y,t_z]^\top\|^2},
\end{equation}
\begin{equation}
 \boldsymbol{t}(\alpha,\beta) = (\cos\alpha, \sin\alpha\cos\beta , \sin\alpha\sin\beta),
\end{equation}
where $\alpha \in [0,\pi]$ and $\beta \in [-\pi,\pi]$; although any $\beta+2k\pi$ gives the same $\boldsymbol{t}$, this constraint is applied for uniqueness.
We shall compare their pros and cons in terms of both network training and fusion. First, it is evident that the unit-norm vector $\boldsymbol{t}$ itself is not a convenient quantity for fusion as it lies in a 2-Sphere manifold. Thus, we seek to fuse the parameters $(t_x,t_y,t_z)$ or $(\alpha,\beta)$. Further, it is also clear that the scale of $(t_x,t_y,t_z)$ is indeterminate, causing the gauge ambiguity and rank-deficient Jacobian. We therefore opt for $(\alpha,\beta)$ as the fusion quantity, i.e. $\boldsymbol{\theta}_t=\{\alpha,\beta\}$. However, due to its circular nature, the warp-around of $\beta$ at $\pm\pi$ leads to discontinuity in the representation; this is not desired in optimization and might cause difficulty in training if the network predicts $\beta$ directly. To address this issue, we designed the network to output $(t_x,t_y,t_z)$ followed by normalization to be of unit-norm, and afterwards we extract $(\alpha,\beta)$ therein, as illustrated in Fig.~\ref{}. 

\noindent \textbf{Circular Fusion}. While the fusion of $\alpha$ remains straightforward, the circular nature slightly complicates the fusion of $\beta$. Ideally, the meaningful fusion is obtained only when $|\beta_c-\beta_g|<\pi$, which could be achieved by letting $\bar\beta_g=\beta_g+2k\pi$ with $k \in \{-1,0,1\}$. The best way to understand this is by looking at a toy example. As illustrated in Fig.~\ref{fig:fusiontoyexample}, depending upon the specific values of $\beta_g$ and $\beta_c$, a direct fusion of the two might yield a solution far from both when $|\beta_c-\beta_g|>\pi$. This is however addressed by fusing $\beta_c$ and $\bar\beta_g$ instead. We term this procedure the circular fusion.

\begin{figure}[t]
	\centering
		\includegraphics[width=0.7\linewidth, trim = 0mm 20mm 0mm 0mm, clip]{Figure/fusiontoyexample.pdf}
	\centering
	\caption{Toy-example illustration of the circle fusion, wherein the fusion is simply defined as averaging. Best viewed in color.}
	\label{fig:fusiontoyexample}
\end{figure}



\noindent \textbf{Rotation}. We consider two minimal 3-parameter representation of rotation---angle-axis representation and Euler angles. The network is designed to regress the angle directly. Although this also faces discontinuity at $\pm\pi$~\cite{}, it however is not as much of a problem as it could be. This is because, rotations between two views in practice are often far from $\pm\pi$ as strong rotation quickly diminishes the overlapping field of view. We observe similar performance from the two representations, but opt for Euler angels since its fusion of roll-pitch-yaw angles has a clearer geometric meaning.


Worth mentioning here is that our pose fusion is related in spirit to translation averaging and rotation averaging (single roation case) in the global SfM lieterature~\cite{}. However, such works typically do not take into account the measurement uncertainty as in our method.

\noindent \textbf{Loss}.


\subsubsection{Self-attention Graph Neural Network}
\noindent \textbf{Network Architecture}. As the network input, we stack the correspondences $(\boldsymbol{x}_i^1,\boldsymbol{x}_i^2)$ between the two views as $\boldsymbol{x}^{12} \in R^{n\times4}$, which is subsequently passed to a MLP for embeding, yielding $\boldsymbol{f}^{(0)}$. Next, $\boldsymbol{f}^{(0)}$ is passed to iterative message passing layers to propagate information between all pairs of correspondences. We adopted the similar network as in SuperGlue~\cite{} for this step due to its extensively proved success. Specifically, in the $l$-th layer, the feature vector $\boldsymbol{f}_i^{l}$ associated with the $i$-th pair of correspondence  is updated as follows
    \boldsymbol{f}_i^{l+1} = \boldsymbol{f}_i^{l} + \text{MLP}([\boldsymbol{f}_i^{l},\boldsymbol{m}_i^l]),
\begin{equation}
\end{equation}
where $[~.~,~.~]$ indicates concatenation. $\boldsymbol{m}_i^l$ denotes the message aggregated from all the correspondences based on the self-attention mechanism~\cite{}. As per the standard procedure, we first define the Query ($\boldsymbol{Q}^l$), Key ($\boldsymbol{K}^l$) and Value ($\boldsymbol{V}^l$) as linear projections of of $\boldsymbol{f}^l$, each with their own learnable parameters shared across all the correspondences. The message $\boldsymbol{m}^l$ is then computed as
\begin{equation}
    \boldsymbol{m}^l = \text{Softmax}(\frac{\boldsymbol{Q}^l\boldsymbol{K}^l^\top}{\sqrt{d_f}})\boldsymbol{V}^l,
\end{equation}
where $d_f$ denotes the feature dimension. The softmax is performed row wise and $\boldsymbol{m}_i^l$ is the $i$-th row of $\boldsymbol{m}^l$.


\noindent \textbf{Why self-attention?} First, it is well-known from classical geometry that each correspondence alone does not determine the camera pose, but rather all the points ($n>=5$) together contribute to the solution. Therefore, the network design should encourage strong interaction between different pairs of correspondences in a tightly-coupled manner. Second, it is also known in classical SfM~\cite{hartley2003multiple} that the spatial distribution of the keypoints leads to different level of perspective effect and this very much affects the well-posedness of motion estimation. 
For instance, one common rule of thumb is that the keypoints should be far from each other and widely spread in the image plane, which effectively makes full use of the field of view and prevenets the degradation of perspective to affine camera model~\cite{}.  Another factor towards preventing affine degradation arises from strong depth variance among different keypoints. Hence, the keypoints are expected to pay varying attentions to the others in order to find the best cousins that together can contribute the most to the final pose estimation. It then becomes clear now that self-attention mechanism naturally stands out as a means to the ends discussed above---enforcing extensive interaction and permits different attentions between each other. Indeed, we empirically observe that self-attention plays a significant role in terms of accuracy.

\noindent \textbf{Remark}. In addition to keypoint locations, attempts were also made to take the descriptors and scores as network input, which nevertheless yields similar performance and hence are omitted.




